3D Feature Prediction for Masked-AutoEncoder-Based Point Cloud Pretraining

Masked autoencoders (MAE) have recently been introduced to 3D self-supervised pretraining for point clouds due to their great success in NLP and computer vision. Unlike MAEs used in the image domain, where the pretext task is to restore features at the masked pixels, such as colors, the existing 3D MAE works reconstruct the missing geometry only, i.e, the location of the masked points. In contrast to previous studies, we advocate that point location recovery is inessential and restoring intrinsic point features is much superior. To this end, we propose to ignore point position reconstruction and recover high-order features at masked points including surface normals and surface variations, through a novel attention-based decoder which is independent of the encoder design. We validate the effectiveness of our pretext task and decoder design using different encoder structures for 3D training and demonstrate the advantages of our pretrained networks on various point cloud analysis tasks.

==> Figures/fig-feavis.tex <==
\begin{figure*}[t]
    \centering
    \begin{overpic}[width=0.652\linewidth]{Images/feavis2}
    \put(4,-3.5){\scriptsize  \textbf{MaskFeat3D}}
    \put(25,-3.5){\scriptsize \textbf{PointBERT}}
    \put(45,-3.5){\scriptsize \textbf{PointMAE}}
    \put(65,-3.5){\scriptsize \textbf{MaskDiscr}}
    \put(85,-3.5){\scriptsize \textbf{MaskSurfel}}
    \end{overpic}
    %\vspace{1pt}
    %\vspace{0.15in}
    \vspace{2mm}
    \caption{\small{\textbf{Feature visualization of different pretrained approaches} including our MaskFeat3D,  PointBERT~\cite{Yu_2022_CVPR}, PointMAE~\cite{Pang2022MaskedAF}, MaskDiscr~\cite{Liu2022maskdis}, MaskSurfel~\cite{zhang2022masked}. Here, note that the absolute colors from different methods are not comparable as their feature spaces are not the same, instead the point color difference from the same method is a good visual measurement for assessing feature discriminativity.
        First row: By comparing the colors of the two front legs, we can see our pretrained network produces more discriminative features than PointBERT and MaskSurfel. Second row: It is clear the features on the different chair legs from our methods, as well as the features of two chair arms, are more discriminative.   } }
    \label{fig:feavis} 
\end{figure*}

==> Tables/augmentation.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{ccc|c}
        \toprule
        rotation & scaling & translation & ScanObjectNN \\ 
        \midrule
        $\surd$ & - & - & 87.0\\
        - & $\surd$ & - & 85.9\\
        $\surd$ & $\surd$ & - & \textbf{87.6}\\
        - & $\surd$ & $\surd$ & 85.1\\
        $\surd$ & $\surd$ & $\surd$ & 86.7 \\   
         
        \bottomrule
    \end{tabular}
    \captionof{table}{Ablation study on pretraining data augmentation.}
    \label{tab:aug}
\end{table}

==> Tables/feature_ablation_2.tex <==
\begin{table}[t]
    \centering
    \setlength\tabcolsep{10pt}
    \resizebox{0.9\linewidth}{!}{  
    \scriptsize
    \begin{tabular}{llc}
        \toprule
      \textbf{Method}  & \textbf{Target Feature} & \textbf{ScanNN}\\
      \midrule
      \multirow{4}{*}{PointMAE}  & position only & 85.2 \\
        & position + normal$^*$ & 85.7 \\
        & position + surface variation$^*$ & 85.9 \\
        & position + normal + variation$^*$ & 86.0 \\
        \midrule
       \multirow{3}{*}{MaskFeat3D} & normal & 86.5 \\
        & surface variation & 87.0\\
         & normal + variation & \textbf{87.7}\\
        % \midrule
        % SDF value & 85.2 \\
        % SDF Gradient & 84.8 \\       
        \bottomrule
    \end{tabular}
    }
    % \vspace{2pt}
    \vspace{-2mm}
    \caption{\small{\textbf{Ablation study on different features.} $^*$ uses position-index matching~\cite{zhang2022masked} for feature loss computation.}}
    %Normal and surface variation, which corresponds to first-order and second-order differential properties, are complementary to each other. Therefore, reconstructing them together yields salient performance gains from reconstructing one of them.}
    \label{tab:feature_ablation}
\end{table}

==> Tables/modelnet40_fewshot.tex <==
\begin{table}[t]
\centering
\setlength\tabcolsep{4pt}
\renewcommand\arraystretch{1}
%\small
\sisetup{
  table-align-uncertainty=true,
  separate-uncertainty=true,
}
%% local redefinitions
\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
\renewrobustcmd{\boldmath}{}
\fontsize{8pt}{11pt}\selectfont

\resizebox{1\linewidth}{!}{
    \scriptsize
\begin{tabular}{lcccc}

\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{5-way}} & \multicolumn{2}{c}{\textbf{10-way}} \\
\cmidrule(lr){2-3}   \cmidrule(lr){4-5}
 & 10-shot & 20-shot & 10-shot & 20-shot \\
\hline
DGCNN$^{\dagger}$~\cite{dgcnn:2019:tog} & $31.6 \pm 2.8$ & $40.8 \pm 4.6$ & $19.9 \pm 2.1$ & $16.9 \pm 1.5$ \\
OcCo~\cite{wang2021unsupervised} & $90.6 \pm 2.8$ & $92.5 \pm 1.9$ & $82.9 \pm 1.3$ & $86.5 \pm 2.2$ \\
CrossPoint~\cite{afham2022crosspoint} & $92.5 \pm 3.0$ & $94.9 \pm 2.1$ & $83.6 \pm 5.3$ & $87.9 \pm 4.2$ \\
\hline
Transformer$^{\dagger}$~\cite{Yu_2022_CVPR} & $87.8 \pm 5.2$ & $93.3 \pm 4.3$ & $84.6 \pm 5.5$ & $89.4 \pm 6.3$ \\
OcCo~\cite{wang2021unsupervised} & $94.0 \pm 3.6$ & $95.9 \pm 2.3$ & $89.4 \pm 5.1$ & $92.4 \pm 4.6$ \\
PointBERT~\cite{Yu_2022_CVPR} & $94.6 \pm 3.1$ & $96.3 \pm 2.7$ & $91.0 \pm 5.4$ & $92.7 \pm 5.1$ \\
MaskDiscr~\cite{Liu2022maskdis} & $95.0 \pm 3.7$ & $97.2 \pm 1.7$ & $91.4 \pm 4.0$ & $93.4 \pm 3.5$ \\
PointMAE~\cite{Pang2022MaskedAF} & $96.3 \pm 2.5$ & $97.8 \pm 1.8$ & $92.6 \pm 4.1$ & $95.0 \pm 3.0$ \\
\rowcolor{gray!20} MaskFeat3D & $\pmb{97.1} \pm \pmb{2.1}$ & $\pmb{98.4} \pm \pmb{1.6}$ &  $\pmb{93.4} \pm \pmb{3.8}$ & $\pmb{95.7} \pm \pmb{3.4}$ \\
\bottomrule
\end{tabular}
}
\label{tab:mn_fewshot}
\vspace{-2mm}
\caption{\small{\textbf{Few-shot classification on ModelNet40.} We report the average accuracy (\%) and standard deviation (\%) of 10 independent experiments.}}
%\vspace{-2mm}
\end{table}

==> Tables/modelnet40_finetune.tex <==
\begin{table}[t]
    \centering

    %
    %\footnotesize
    \begin{tabular}{lc}
        \toprule
        \textbf{Method} & \textbf{ModelNet40} \\
        \midrule
        Transformer$^{\dagger}$ ~\cite{Yu_2022_CVPR}     & 91.4 \\
        PointBERT~\cite{Yu_2022_CVPR}    & 93.2 \\
        MaskDiscr~\cite{Liu2022maskdis}  & 93.8 \\
        MaskSurfel~\cite{zhang2022masked} & 93.6 \\
        PointMAE~\cite{Pang2022MaskedAF} & 93.8 \\
        \rowcolor{gray!20}MaskFeat3D    & \textbf{93.9} \\
        \bottomrule
    \end{tabular}
    % \vspace{5pt}
    \vspace{-2mm}
    \caption{\small{\textbf{Shape classification fine-tuned on ModelNet40.} All the methods use the same transformer backbone architecture. $^{\dagger}$ represents the \textit{from scratch} results and all other methods represent the \textit{fine-tuning} results using pretrained weights.}}
    \label{tab:modelnet40}
    %\vspace{-3pt}
\end{table}



==> Tables/pointnext_ablation.tex <==
\begin{wraptable}[19]{r}{0.56\linewidth}
    \centering
    \footnotesize
    \setlength\tabcolsep{3pt}
    \begin{tabular}{lccc}
        \toprule
       \textbf{cases} &  \textbf{channel}(c) & \textbf{ScanObjectNN} & \textbf{ShapeNetPart}\\
       \midrule
      \small{Scratch} & 3 & 87.1 & 85.6\\
      \small{MaskFeat3D} & 3 & 88.0 & 86.8\\
      \midrule
      \small{Scratch} & 4 & 88.1 & 86.0 \\
      \small{MaskFeat3D} & 4 & \textbf{88.6} & 87.0 \\
      \midrule
      \small{Scratch} & 7 & - & 87.1\\
      \small{MaskFeat3D} & 7 & - & \textbf{87.4}\\
        \bottomrule
    \end{tabular}
    \captionof{table}{\textbf{Comparison of PointNeXt backbone under different input channel numbers.}    `Scratch' means training from scratch. `MaskFeat3D' means fine-tuning on the pretrained weight of our model. We report overall accuracy for ScanObjectNN PB-T50-RS split, and ins. mIoU for ShapeNetPart task. Channel $c = 3$ means only using position. $c = 4$ uses position and height information. $c = 7$ uses position, height, and point normal. Since ScanObjectNN dataset does not contain point normal labels, we leave $c = 7$ entries blank.}
    \label{tab:pointnext_ablation} 
\end{wraptable}

==> Tables/s3dis_2.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{lcccc}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Sem Seg}}& \multicolumn{2}{c}{\textbf{Detection}} \\ 
      \cmidrule(lr){2-3}   \cmidrule(lr){4-5} &  mIoU & OA & mAP$_{0.25}$ & mAP$_{0.5}$ \\
        \midrule
        PointNet~\cite{qi2017pointnet} & 41.1 & 49.0 &  - & - \\ 
        PointNet++~\cite{qi2017pointnet++} & 53.5 & 67.1 & 46.1 & 24.5 \\
        PointCNN~\cite{pointcnn} & 57.3 & 85.9 &  - & - \\
        GSDN~\cite{gwak2020generative} & - & - & 47.8 & 25.1 \\
        DGCNN~\cite{dgcnn:2019:tog} & 47.9 & 83.6 & - & - \\
        PointTrans~\cite{pointr} & 70.4 & 90.8 &  - & - \\
        FCAF3D~\cite{rukhovich2022fcaf3d} & 65.4 & 89.1 & 66.7 & 45.9 \\
        PointNeXt~\cite{PointNeXt} & 70.8 & 90.7 &  - & - \\
        \midrule
        Point-MAE & 60.8 & 69.9 & - & - \\
        Point-M2AE~\cite{zhang2022point} & - & - & 50.1 & 33.2 \\
        \rowcolor{gray!20}MaskFeat3D & \textbf{71.7} & \textbf{91.7} & \textbf{71.6} & \textbf{49.2} \\
        \bottomrule
    \end{tabular}
    \vspace{2pt}
    \caption{\small{\textbf{Area 5 Semantic segmentation and detection results on S3DIS.}}}
    \label{tab:s3dis} 
    %\vspace{-4mm}
\end{table}



==> Tables/s3dis_3.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabular}{lcccc}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Sem Seg}}& \multicolumn{2}{c}{\textbf{Detection}} \\ 
      \cmidrule(lr){2-3}   \cmidrule(lr){4-5} &  mIoU & OA & mAP$_{0.25}$ & mAP$_{0.5}$ \\
        %\midrule
        %PointNet~\cite{qi2017pointnet} & 41.1 & 49.0 &  - & - \\ 
        %PointNet++~\cite{qi2017pointnet++} & 53.5 & 67.1 & 46.1 & 24.5 \\
        %PointCNN~\cite{pointcnn} & 57.3 & 85.9 &  - & - \\
        %GSDN~\cite{gwak2020generative} & - & - & 47.8 & 25.1 \\
        %DGCNN~\cite{dgcnn:2019:tog} & 47.9 & 83.6 & - & - \\
       % PointTrans~\cite{pointr} & 70.4 & 90.8 &  - & - \\
        %Point-MAE & 60.8 & 69.9 & - & - \\
        %Point-M2AE~\cite{zhang2022point} & - & - & 50.1 & 33.2 \\
        \midrule
        PointNeXt$^{\dagger}$~\cite{PointNeXt} & 70.8 & 90.7 &  - & - \\
        MaskFeat3D & \textbf{71.7} & \textbf{91.7} & - & - \\
        \midrule
        FCAF3D$^{\dagger}$~\cite{rukhovich2022fcaf3d} & - & - & 66.7 & 45.9 \\
        MaskFeat3D & - & - & \textbf{71.6} & \textbf{49.2} \\
        \bottomrule
    \end{tabular}
    %\vspace{2pt}
    \vspace{-2mm}
    \caption{\small{\textbf{Area 5 Semantic segmentation and detection results on S3DIS.} $^{\dagger}$ represents the \textit{from scratch} results and MaskFeat3D in the same section represents the \textit{fine-tuning} results using pretrained weights under same backbone.}}
    \label{tab:s3dis} 
    \vspace{-6mm}
\end{table}



==> Tables/shape_segmentation.tex <==
\begin{table}
    \centering
    %\setlength\tabcolsep{20pt}
    \begin{tabular}{l|ll}
        \toprule
        \textbf{Method} & ins. mIoU & cls. mIoU\\
        \midrule
         PointNet & 83.7 & 80.4\\
        DGCNN & 85.2 & 82.3\\
        PointNet++ & 85.1 & 81.9\\
        PointTransform & 86.6 & 83.7\\
        PointMLP & 86.1 & 84.6 \\
        Stratified & 86.6 & 85.1 \\
        \midrule
        %Jigsaw\citep{sauder2019self} & 92.4\% \\
        
        PointViT & 85.1 & 83.4 \\
        $\text{[S]}$Point-BERT & 85.6 & 84.1\\
        $\text{[S]}$MaskPoint & 86.0 & 84.4 \\
        $\text{[S]}$Point-MAE & 86.1 & - \\
        \rowcolor{gray!20}$\text{[S]}$ MaskFeat & \textbf{86.2} $\pm$ 0.0\textcolor[rgb]{0,0.6,0}{(+0.1)}& \textbf{84.6} $\pm$ 0.1\textcolor[rgb]{0,0.6,0}{(+0.3)} \\
        \midrule
        MinkowskiNet & - & -\\
        \rowcolor{gray!20}$\text{[S]}$ MaskFeat & - & -\\
        \midrule
        PointNeXt & 87.0 $\pm$ 0.1 & 85.2 $\pm$ 0.1\\
        \rowcolor{gray!20}$\text{[S]}$ MaskFeat & \textbf{87.3} $\pm$ 0.1\textcolor[rgb]{0,0.6,0}{(+0.3)} & \textbf{85.3} $\pm$ 0.1 \textcolor[rgb]{0,0.6,0}{(+0.1)}\\
        \bottomrule
    \end{tabular}
    \captionof{table}{ShapeNetPart Segmentation.}
    \label{tab:sbnn}
\end{table}

==> Tables/supp_ablation.tex <==
\begin{table*}[t]
%\scriptsize
\setlength\tabcolsep{10pt}
\begin{subtable}[t]{.3\textwidth}
\centering  
%\scriptsize
\footnotesize
\caption{\footnotesize \textbf{Neighborhood size}}
    \begin{tabular}{cc}
    \toprule
     r & ScanObjectNN \\
        \midrule
        0.05 & 86.6 \\
        0.07 & 87.0 \\
        \rowcolor{gray!20} 0.1 & \textbf{87.7} \\
        0.2 & 86.8 \\
        \bottomrule
    \end{tabular}
     \label{tab:sv_ablation}
\end{subtable}
 %\hfill
 \hspace*{0.017\textwidth}
\begin{subtable}[t]{.3\textwidth}
\centering  
%\scriptsize
\footnotesize
\caption{\footnotesize \textbf{Number $k$ in FPS}} 
\begin{tabular}{cc}
\toprule
        \# $k$ & ScanObjectNN \\ 
        \midrule
        8 & 87.4 \\
        16 & 87.4 \\
        \rowcolor{gray!20} 32 & \textbf{87.7} \\
        64 & 87.6 \\
        128 & 87.6 \\
        \bottomrule
    \end{tabular}
    \label{tab:fps}
\end{subtable}
 %\hfill 
\begin{subtable}[t]{.33\textwidth}
\centering  
\footnotesize
\caption{\footnotesize \textbf{Mask region}} 
    \begin{tabular}{cc}
    \toprule
     region & ScanObjectNN \\
        \midrule
        \rowcolor{gray!20} masked only & \textbf{87.7} \\
        all points & 86.8 \\
        \bottomrule
    \end{tabular}
    \label{tab:unmasked}
\end{subtable}

\caption{\small{\textbf{More ablation studies of our design choices}. Please refer to \cref{sec:supp-ablation} for more details.}}
\label{tab:ablation} \vspace{-5mm}
\end{table*}


==> Tables/supp_fps.tex <==
\begin{table}[h]
    \centering
    %\footnotesize
    \vspace{-7pt}
    \scriptsize
    \begin{tabular}{cccccc}
        %\toprule
        \# $k$ & 8 & 16 & 32 & 64 & 128 \\
        \midrule
        ScanObjectNN & 87.4 & 87.4 & \textbf{87.7} & 87.6 & 87.6 \\
        %\bottomrule
    \end{tabular}
    %\caption{}
    \vspace{-12pt}
    \label{tab:fps} 
\end{table}



==> Tables/supp_modelnet.tex <==
\begin{table*}[t]
\small
\begin{minipage}[b]{.45\linewidth}
    \centering
   \setlength\tabcolsep{5pt}% 调整列间距
    \begin{tabular}{lc}
        \toprule
        \textbf{Method} & \textbf{ModelNet40} \\
        \midrule
        PointViT$^{\dagger}$ ~\cite{Yu_2022_CVPR}     & 91.4 \\
        PointBERT~\cite{Yu_2022_CVPR}    & 93.2 \\
        MaskDiscr~\cite{Liu2022maskdis}  & 93.8 \\
        MaskSurfel~\cite{zhang2022masked} & 93.6 \\
        PointMAE~\cite{Pang2022MaskedAF} & 93.8 \\
        \rowcolor{gray!20}MaskFeat3D (PointViT)    & \textbf{93.9} \\
        \bottomrule
    \end{tabular}
    \captionof{table}{\small{\textbf{Shape classification fine-tuned on ModelNet40.} All the methods use the same transformer backbone architecture. $^{\dagger}$ represents the \textit{from scratch} results and all other methods represent the \textit{fine-tuning} results using pretrained weights.}}
    \label{tab:modelnet40}
\end{minipage}\hspace{.02\linewidth}
\begin{minipage}[b]{.5\linewidth}
 \setlength\tabcolsep{5pt}
    \begin{tabular}{lc}
        \toprule
        \textbf{Method} & \textbf{Acc. (\%)} \\
        \midrule
        %Random &  60.2\% \\
        3D-GAN~\cite{wu2016learning}  & 83.3 \\
        Latent-GAN~\cite{achlioptas2018learning} & 85.7 \\
        SO-Net~\cite{li2018so} & 87.3 \\
        MAP-VAE~\cite{han2019multi} & 88.4 \\
        Jigsaw~\cite{sauder2019self} & 84.1 \\
        FoldingNet~\cite{yang2018foldingnet} & 88.4 \\
        DGCNN + OcCo~\cite{wang2021unsupervised} & 89.7 \\
        DGCNN + STRL~\cite{huang2021spatio} & 90.9 \\
        \midrule 
        PointViT + OcCo$^*$~\cite{wang2021unsupervised} & 89.6 \\
        PointBERT~\cite{Yu_2022_CVPR}$^*$ & 87.4 \\
        %MaskDiscr$^*$ & \\
        PointMAE~\cite{Pang2022MaskedAF}$^*$ & 88.5 \\
        \rowcolor{gray!20}MaskFeat3D (PointViT) $^*$ & \textbf{91.1}\\
        
        \bottomrule
    \end{tabular}
    \captionof{table}{\small{\textbf{Linear evaluation for shape classification on ModelNet40}. This task is sensitive to the encoder backbone. Different * methods use the same Transformer encoder backbone.}}
    \label{tab:svm}
\end{minipage}
\end{table*}

==> Tables/supp_unmasked.tex <==
\begin{table}[h]
    \centering
    \scriptsize
    %\footnotesize
    \vspace{-8pt}
    \begin{tabular}{ccc}
        %\toprule
         & \textbf{masked only} & \textbf{all points} \\
        \midrule
        ScanObjectNN (PB-T50-RS) & \textbf{87.7} & 86.8 \\
        %\bottomrule
    \end{tabular}
    %\caption{}
    \vspace{-12pt}
    \label{tab:supp-unmask}
    
\end{table}



==> Tables/sv_ablation.tex <==
\begin{table}
    \centering
    \begin{tabular}{cc}
    \toprule
     \textbf{r} & \textbf{ScanObjectNN} (OA(\%)) \\
        \midrule
        0.05 & 86.6 \\
        0.07 & 87.0 \\
        \rowcolor{gray!20} 0.1 & 87.7 \\
        0.2 & 86.8 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Ablation study on the neighborhood size} $r$ in shape surface variation. We utilize the ViT-based encoder and present the overall accuracy on the ScanObjectNN PB-T50-RS split.}
    \label{tab:sv_ablation}
\end{table}

==> Tables/svm.tex <==
\begin{table}
    \centering
    \setlength\tabcolsep{20pt} 
    \resizebox{1.\linewidth}{!}{
    \footnotesize
    \begin{tabular}{lc}
        \toprule
        \textbf{Method} & \textbf{Acc. (\%)} \\
        \midrule
        %Random &  60.2\% \\
        3D-GAN~\cite{wu2016learning}  & 83.3 \\
        Latent-GAN~\cite{achlioptas2018learning} & 85.7 \\
        SO-Net~\cite{li2018so} & 87.3 \\
        MAP-VAE~\cite{han2019multi} & 88.4 \\
        Jigsaw~\cite{sauder2019self} & 84.1 \\
        FoldingNet~\cite{yang2018foldingnet} & 88.4 \\
        DGCNN + OcCo~\cite{wang2021unsupervised} & 89.7 \\
        DGCNN + STRL~\cite{huang2021spatio} & 90.9 \\
        DGCNN + IAE~\cite{yan2022implicit} & 92.1 \\
        Point-M2AE~\cite{zhang2022point} & \underline{92.9} \\
        \midrule 
        Transformer + OcCo$^*$~\cite{wang2021unsupervised} & 89.6 \\
        PointBERT~\cite{Yu_2022_CVPR}$^*$ & 87.4 \\
        %MaskDiscr$^*$ & \\
        PointMAE~\cite{Pang2022MaskedAF}$^*$ & 88.5 \\
        \rowcolor{gray!20}MaskFeat3D$^*$ & \textbf{91.1}\\
        
        \bottomrule
    \end{tabular}
    }
    % \vspace{5pt}
    \vspace{-2mm}
    \caption{\small{\textbf{Linear evaluation for shape classification on ModelNet40}. This task is sensitive to the encoder backbone. Different * methods use the same Transformer encoder backbone.}} 
    \vspace{-2mm}
    \label{tab:svm}
\end{table}
